Physics-Informed Neural Network for the Transient Diffusivity Equation in Reservoir Engineering

Physics-Informed machine learning models have recently emerged with some interesting and unique features that can be applied to reservoir engineering. In particular, physics-informed neural networks (PINN) leverage the fact that neural networks are a type of universal function approximators that can embed the knowledge of any physical laws that govern a given data-set in the learning process, and can be described by partial differential equations. The transient diffusivity equation is a fundamental equation in reservoir engineering and the general solution to this equation forms the basis for Pressure Transient Analysis (PTA). The diffusivity equation is derived by combining three physical principles, the continuity equation, Darcy's equation, and the equation of state for a slightly compressible liquid. Obtaining general solutions to this equation is imperative to understand flow regimes in porous media. Analytical solutions of the transient diffusivity equation are usually hard to obtain due to the stiff nature of the equation caused by the steep gradients of the pressure near the well. In this work we apply physics-informed neural networks to the one and two dimensional diffusivity equation and demonstrate that decomposing the space domain into very few subdomains can overcome the stiffness problem of the equation. Additionally, we demonstrate that the inverse capabilities of PINNs can estimate missing physics such as permeability and distance from sealing boundary similar to buildup tests without shutting in the well.

==> comments.tex <==
\begin{comment}
    A better understanding on the distribution of error for each training run can be obtained by analysing Table \ref{table:burgers_results}.
    \begin{table}[ht]
        \centering
        \begin{tabular}{ cccc } 
            \toprule
                       & \multicolumn{3}{c}{L2 Error}\\
            \cline{2-4}
                Method & Median & Mean & Standard Deviation \\
            \midrule
                PINN with a priori AV & 6.1\%  & 6.1\%  & 0.1\% \\ 
                PINN-ALAV             &    \% &     \%  &    \% \\ 
             \bottomrule
        \end{tabular}
        \caption{Methods prediction error on Burger's Equation calculated over 20 training runs}
        \label{table:burgers_results}
    \end{table}
\end{comment}




\begin{comment}
    The results presented until this point for PINN-ALAV used $\alpha_{visc} = 1.0$. Table \ref{table:burgers_results} shows that PINN-ALAV has an error mean and standard deviation considerably higher than the other methods. To reduce this error we tried to vary the value of  $\alpha_{visc}$ and also change the artificial viscosity loss function that was define in terms of a mean square error (eq. \ref{eq:pinn_loss_alav}) and we are going to test also L1 and L2 norms. Then the respective loss function are defined as $\mathcal{L}_{visc-L1} = \norm{\epsilon(\vb*{x}, t)}_1$ and $\mathcal{L}_{visc-L2} = \norm{\epsilon(\vb*{x}, t)}_2$.
    
    \begin{figure}
        \begin{subfigure}{0.31\textwidth}
            \includegraphics[width=\linewidth]{figures/burgers_diffLossMult_MSE.pdf}
            \caption{MSE}
            \label{fig:burgers_alpha_visc_norms_mse}
        \end{subfigure}
        \hspace*{\fill}
        \begin{subfigure}{0.31\textwidth}
            \includegraphics[width=\linewidth]{figures/burgers_diffLossMult_L2.pdf}
            \caption{L2}
            \label{fig:burgers_alpha_visc_norms_l2}
        \end{subfigure}
        \hspace*{\fill}
        \begin{subfigure}{0.31\textwidth}
            \includegraphics[width=\linewidth]{figures/burgers_diffLossMult_L1.pdf}
            \caption{L1}
            \label{fig:burgers_alpha_visc_norms_l1}
        \end{subfigure}
        \caption{Prediction error evaluation for different values of $\alpha_{visc}$ and different types of artificial viscosity loss function (MSE, L2 and L1)}
        \label{fig:burgers_alpha_visc_norms}
    \end{figure}
    
    Figure \ref{fig:burgers_alpha_visc_norms} shows that MSE and L2 artificial viscosity loss functions have a same error behaviour when changing $\alpha_{visc}$. Interesting to note that L1 artificial viscosity loss has a different behaviour, showing that the minimum error happens when using $\alpha_{visc} = 1.0\times 10^{-3}$. 
    The artificial viscosity map for L1 artificial viscosity loss function is shown on Figure \ref{fig:burgers_viscosity_map_l1} where is possible to conclude that more values on the regions we expect to have zero artificial viscosity are indeed closer to zero. When comparing this figure with their counterpart using MSE (Figure \ref{fig:burgers_viscosity_map}) it is possible to see that the histograms confirm this observation, since there are less values in that region close to zero but not zero.
    
    \begin{figure}
        \centering
        \includegraphics[width=0.6\linewidth]{figures/burgers_viscosity_map_l1.pdf}
        \caption{Artificial viscosity map and distribution for Burger's equation using PINN-ALAV with L1 artificial viscosity loss function.}
        \label{fig:burgers_viscosity_map_l1}
    \end{figure}
\end{comment}

\begin{comment}
    \subsection{PINN with Adaptive Artificial Viscosity - PINN-AAV}
    Like in \cite{fuks_limitations_2020}, the idea here is to use the artificial viscosity, but instead of setting its value a priori, this will be a parameters learned along the learning process. First the residual equation is redefined to:
    \begin{align}
        r(\vb*{x}, t, \vb*{w}, \epsilon) = 
        \pdv{u(\vb*{x},t, \vb*{w})}{t} + \mathcal{N}(u(\vb*{x},t, \vb*{w})) - \epsilon\pdv[2]{u(\vb*{x},t, \vb*{w})}{x} ,
    \end{align}
    and consequentially the residual loss function and total loss function will also be a function of the artificial viscosity, $\mathcal{L}_r = \mathcal{L}_r(\vb*{w},\epsilon)$ and $\mathcal{L} = \mathcal{L}(\vb*{w},\epsilon)$. To provide constrains to the learnable variable $\epsilon$, an additional loss function term was introduced:
    \begin{equation}
        \mathcal{L}_{visc}(\epsilon) = \textrm{MSE}(\epsilon, 0.0)
    \end{equation}
    and the total loss function is now defined as:
    \begin{equation}
        \mathcal{L}(\vb*{w}, \epsilon) = \mathcal{L}_r(\vb*{w}, \epsilon) + \mathcal{L}_b(\vb*{w}) + \mathcal{L}_0(\vb*{w}) + \mathcal{L}_{visc}(\epsilon). \label{eq:pinn_loss_aav}
    \end{equation}
\end{comment}









\subsubsection{Convex fractional flow}
The solution of the Buckley-Leverett problem (Eq. \ref{eq:bl_eq_system}) when a convex fraction flow function is used presents a shock along with all domains (Figure \ref{fig:ff_convex_output}). The fractional flow function used in this section is:
\begin{equation}
    f_w(S_w) = S_w^2 \label{eq:bl_convex_ff}
\end{equation}

As mentioned previously the presence of shocks in the solution increases the difficulty that numerical methods and also methods like PINN's face while solving these problems. \cite{fuks_limitations_2020} showed that this problem can be solved by PINN's adding an artificial viscosity with a predefined value. In Figure \ref{fig:bl_convex_results} a comparison between this method and methods PINN-AAV and PINN-ALAV to learn the artificial viscosity value is presented. It is possible to confirm that the methods proposed here provide a good match with the analytical solution.
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/burger_pinn_alav.pdf}
    \caption{Buckley-Leverett problem with a convex fractional flow function solved by PINN-AAV and PINN-ALAV}
    \label{fig:bl_convex_results}
\end{figure}

In Table \ref{table:bl_convex_results} the mean and standard deviation of L2 error over 20 training runs are presented.

\begin{table}[h!]
    \centering
    \begin{tabular}{ c|c|c } 
        \hline
            Method & L2 Error Mean & L2 Error Standard Deviation \\
        \hline
            PINN with a priori AV &  &  \\ 
            PINN-AAV  &  &  \\ 
            PINN-ALAV & 0 & 0 \\ 
         \hline
    \end{tabular}
    \caption{Methods prediction error on Buckley-Leverett with convex fractional flow function}
    \label{table:bl_convex_results}
\end{table}














\subsubsection{Concave fractional flow function}
The concave flux function is defined as:
\begin{equation}
    f_w(S_w) = \frac{S_w}{S_w + \frac{1-S_w}{M}}
\end{equation}
where $M=\frac{\mu_o}{\mu_w}$ is the viscosity ratio.

\cite{fuks_limitations_2020} showed that baseline PINNs with no artificial viscosity can be used to obtain a good solution for this type of fractional flow function. Here we confirm that and showed that we can obtain similar results by using PINN-ALAV. At first glance, one can conclude that no gain is obtained by using PINN-ALAV, however here we are showing that we can use the localized adaptive diffusion coefficient without really checking the behavior of the fractional flow curve. If discontinuities are present, the artificial viscosity is used only where is necessary. In the case where no discontinuity happens on the solution domain, the artificial viscosity values remain zero on the whole solution domain. The results of PINN-ALAV and the baseline PINNs are presented in Figure \ref{fig:bl_concave_m2}.
\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth]{figures/bl_concave_m2.pdf}
	\caption{Concave fractional flow with $M = 2$}
	\label{fig:bl_concave_m2}
\end{figure}

A map of artificial viscosity values is presented in Figure xxx to confirm that all values on the solution domain are zero.
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/bl_concave_m2_alav_viscosity_map.pdf}
    \caption{PINN-ALAV artificial viscosity map for Buckley-Leverett problem with concave fraction flow $M=2$}
    \label{fig:bl_concave_m2_alav_viscosity_map}
\end{figure}

Similar results were obtained for $M=3$ (Figure \ref{fig:bl_concave_m3}) where both baseline PINNs with no diffusion coefficient and PINN-ALAV provided similar results. 
\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth]{figures/bl_concave_m3.pdf}
	\caption{Concave fractional flow with $M = 3$}
	\label{fig:bl_concave_m3}
\end{figure}














